Bayesian Uncertainty Directed Trial Designs

Most Bayesian response-adaptive designs unbalance randomization rates towards the most promising arms with the goal of increasing the number of positive treatment outcomes during the study, even though the primary aim of the trial is different. We discuss Bayesian uncertainty directed designs (BUD), a class of Bayesian designs in which the investigator specifies an information measure tailored to the experiment. All decisions during the trial are selected to optimize the available information at the end of the study. The approach can be applied to several designs, ranging from early stage multi-arm trials to biomarker-driven and multi-endpoint studies. We discuss the asymptotic limit of the patient allocation proportion to treatments, and illustrate the finite-sample operating characteristics of BUD designs through examples, including multi-arm trials, biomarker-stratified trials, and trials with multiple co-primary endpoints.

==> TableMAMS2.tex <==
\begin{table}[ht]
\centering
\small


 \renewcommand{\arraystretch}{1.1}% Wider
\begin{tabular}{| r  r  |  rrr |  rrr | rrr |}
\hline

 & \textcolor{black}{Control} &  \multicolumn{3}{c|}{Arm 1} & \multicolumn{3}{c|}{Arm 2} & \multicolumn{3}{c|}{Arm 3} \\
 
 \textbf{Design}    & ESS (SD) 
 & \multicolumn{3}{c|}{ {\footnotesize  ESS (SD)  Power  MSE}}  
 & \multicolumn{3}{c|}{ {\footnotesize ESS (SD)  Power  MSE}}  
 & \multicolumn{3}{c|}{ {\footnotesize ESS (SD)  Power  MSE}}    \\
 \hline
% \hline
&  \multicolumn{10}{l|}{\textbf{Scenario 1}: no effective arm 
$(\theta_0, \theta_1,\theta_2,\theta_3)=(0.4 ,0.4,0.4,0.4)$}\\
  % \hline
  BR        &  84 (8)   & 84 (08) & 04.0 & 5.89 & 84 (8) & 04.1 & 5.86 & 84 (8) & 03.2 & 5.74 \\ 
  BUD     & 118 (3)  & 73 (03) & 03.8 & {\bf 5.44} & 73 (3) & 03.8 & {\bf5.43} & 73 (3) & 04.0 & {\bf5.52} \\ 
  BAR     &  97 (8)   & 80 (21) & 03.9 & 7.33 & 79 (21) & 03.6 & 7.30 & 80 (21) & 03.8 & 7.28 \\ 
  BAR2  & 84  (23) & 84 (22) & 03.9 & 7.26 & 84 (22) & 04.0 & 7.17 & 84 (23) & 04.2 & 7.37 \\
   
  DBCD1 & 84 (4) & 84 (4) & 03.8 & 5.93 & 84 (4) & 03.8 & 5.85 & 84 (4) & 03.6 & 5.82 \\ 
  DBCD2 & 84 (6) & 84 (6) & 03.6 & 5.89 & 84 (6) & 03.9 & 5.92 & 84 (6) & 03.5 & 5.82 \\ 
 \hline
  
& \multicolumn{10}{l|}{\textbf{Scenario 2:}  one superior arm $(\theta_0, \theta_1,\theta_2,\theta_3)=(\textbf{0.4} ,\textbf{0.6},0.4,0.4)$}\\
 %  \hline
  BR        & 85 (8) & 84 (8) & 78.6 & 5.75 & 83 (8) & 04.2 & 5.75 & 84 (8) & 03.3 & 5.80 \\ 
  BUD     & 118 (3) & 73 (3) & 82.2 & 5.48 & 73 (3) & 03.6 & {\bf5.46} & 73 (3) & 03.8 & {\bf5.40} \\ 
  BAR     & 100 (10) & 103 (14) & {\bf 87.5} & {\bf 4.89} & 67 (18) & 03.2 & 7.65 & 66 (18) & 03.6 & 7.96 \\ 
  BAR2  & 58  (17 ) & 161 (28) & 85.1 & 6.80 & 58  (17) & 3.4 &  9.80 & 58  (17)  & 3.5  & 9.65\\
  DBCD1 & 84 (4)    & 84 (4)     & 79.8 & 5.99 & 84 (4) & 03.9 & 6.07 & 84 (4) & 04.0 & 6.02 \\ 
  DBCD2 & 80 (6)    & 97 (6)     & 81.2 & 5.63 & 80 (6) & 03.4 & 6.16 & 80 (6) & 03.7 & 6.09 \\ 
    \hline
    
& \multicolumn{10}{l|}{\textbf{Scenario 3:} one superior and one inferior arm  $(\theta_0, \theta_1,\theta_2,\theta_3)=(\textbf{0.4} ,\textbf{0.6},0.4,0.2)$}\\
 %\hline
 BR & 84 (8) & 84 (8) & 78.9 & 5.92 & 84 (8) & 03.6 & 5.70 & 84 (8) & 0.00 & 4.72 \\ 
  BUD & 122 (4) & 75 (3) & 84.3 & 5.10 & 75 (3) & 03.6 & {\bf5.22} & 63 (5) & 0.00 & {\bf4.68} \\ 
  BAR & 111 (10) & 117 (13) & {\bf 90.6} & {\bf4.40} & 75 (20) & 04.0 & 7.22 & 32 (11) & 0.00 & 8.12 \\ 
  BAR2 & 62(18) & 180 (27)& 88.2  & 6.24 & 62 (18)  & 3.4  & 9.04  & 31 (8) & 0.0 & 9.95 \\
   
  DBCD1 & 88 (4) & 88 (4) & 81.1 & 5.69 & 88 (4) & 03.7 & 5.66 & 72 (7) & 0.00 & 5.20 \\ 
  DBCD2 & 85 (7) & 104 (6) & 83.8 & 5.25 & 85 (7) & 03.8 & 5.95 & 61 (8) & 0.00 & 5.76 \\ 
  \hline
& \multicolumn{10}{l|}{\textbf{Scenario 4:} three superior arms  $(\theta_0, \theta_1,\theta_2,\theta_3)=(\textbf{\textcolor{black}{0.4}},\textbf{0.6},\textbf{0.65},\textbf{0.7})$}\\
 %\hline
 BR & 84 (8) & 85 (8) & 79.4 & 5.89 & 84 (8) &   92.5 & 5.86 & 84 (8)   & 98.6 & 5.74 \\ 
  BUD & 120 (3) & 74 (3) & {\bf 83.6} & {\bf5.34} & 72 (3) & {\bf 95.1} & {\bf5.18} & 70 (4)  & {\bf 99.1} & {\bf5.14} \\ 
  BAR & 90 (4) & 80 (9) & 79.2 & 7.33 & 82 (8) & 93.4 & 7.30 & 83 (8)   & 98.6 & 7.28 \\ 
  BAR2 & 35 (10) &  75  (22) & 55.1 & 11.94 & 96  (26) & 78.8 & 10.77 & 130  (29) & 95.3 & 9.87\\
  DBCD1 & 86 (4) & 86 (4) & 80.4 & 5.93 & 84 (5) & 94.0 & 5.85 & 80 (5) & 98.6 & 5.82 \\ 
  DBCD2 & 70 (6) & 85 (5) & 75.8 & 5.89 & 89 (5) & 91.7 & 5.92 & 92 (5) & 98.4 & 5.82 \\       
  \hline

\end{tabular}
%\end{table}

\caption{\small 
Expected sample size (ESS), standard deviation (SD), power and mean squared error (MSE), for each experimental arm in a 4-arm trial with $336$ patients using 
either
balanced randomization (BR),
Bayesian uncertainty directed (BUD) sampling,
{two versions of Bayesian adaptive randomization (BAR and BAR2) 
described in \cite{trippa2012bayesian} (BAR) and  \cite{thall2007practical} (BAR2),}
and two versions of the  doubly adaptive biased coin design (DBCB1 and DBCD2).
The MSE is scaled by a factor of $10^3$.
}  
\label{TAB1}
\end{table}




